Crime scene classification from skeletal trajectory analysis in surveillance settings

Video anomaly analysis is a core task actively pursued in the field of computer vision, with applications extending to real-world crime detection in surveillance footage. In this work, we address the task of human-related crime classification. In our proposed approach, the human body in video frames, represented as skeletal joints trajectories, is used as the main source of exploration. First, we introduce the significance of extending the ground truth labels for HR-Crime dataset and hence, propose a supervised and unsupervised methodology to generate trajectory-level ground truth labels. Next, given the availability of the trajectory-level ground truth, we introduce a trajectory-based crime classification framework. Ablation studies are conducted with various architectures and feature fusion strategies for the representation of the human trajectories. The conducted experiments demonstrate the feasibility of the task and pave the path for further research in the field.

==> baseline_results_table.tex <==
\begin{table}[h]

\centering
\resizebox{.5\textwidth}{!}{
\begin{tabular}{ll|c}
\multicolumn{2}{l|}{Dataset} & AUROC \\ 
\hline \hline
\multicolumn{2}{l}{\textit{Baseline\_M1: New baseline for HR-ShanghaiTech}}\\
\hline
\multicolumn{2}{l|}{HR-ShanghaiTech (de novo)} & \textbf{0.735}  \\
\hline
\multicolumn{2}{l}{\textit{Baseline\_M2, Baseline\_M3: Fine-tuning MPED-RNN on HR-Crime}}\\
\hline
\multicolumn{2}{l|}{HR-Crime (de novo)} & \textbf{0.603}  \\
\multicolumn{2}{l|}{HR-ShanghaiTech (fine-tuned)} & 0.588  \\
\hline
\multicolumn{2}{l}{\textit{Baseline\_M4: MPED-RNN on HR-Crime}}\\
\hline
\multicolumn{2}{l}{HR-ShanghaiTech (pre-trained) \cite{mpedrnn}} & 0.535\\
    \end{tabular}}
\caption{Baseline results for the HR-ShanghaiTech and HR-Crime datasets using MPED-RNN models.}
\label{tab:baseline_results}
\end{table}

==> bibliowithIEEE.tex <==
@article{anomaly_survey,
  title={Anomaly detection: A survey},
  author={Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  journal={ACM computing surveys},
  volume={41},
  number={3},
  pages={1--58},
  year={2009},
  publisher={ACM New York, NY, USA}
}

@article{violence1,
  title={Violence detection in videos for an intelligent surveillance system using MoBSIFT and movement filtering algorithm},
  author={Febin, IP and Jayasree, K and Joy, Preetha Theresa},
  journal={Pattern Analysis and Applications},
  pages={1--13},
  year={2019},
  publisher={Springer}
}

@article{violence2,
  title={A new method for violence detection in surveillance scenes},
  author={Zhang, Tao and Yang, Zhijie and Jia, Wenjing and Yang, Baoqing and Yang, Jie and He, Xiangjian},
  journal={Multimedia Tools and Applications},
  volume={75},
  number={12},
  pages={7327--7349},
  year={2016},
  publisher={Springer}
}

@article{violence3,
  title={Human violence recognition and detection in surveillance videos},
  author={Bilinski, Piotr and Bremond, Francois},
  journal={IEEE Int. Conference on Advanced Video and Signal Based Surveillance (AVSS)},
  pages={30--36},
  year={2016},
  organization={IEEE}
}

@article{car1,
  title={Motion interaction field for accident detection in traffic surveillance video},
  author={Yun, Kimin and Jeong, Hawook and Yi, Kwang Moo and Kim, Soo Wan and Choi, Jin Young},
  journal={Int. Conference on Pattern Recognition},
  pages={3062--3067},
  year={2014},
  organization={IEEE}
}

@article{car2,
  title={Anomaly detection in traffic surveillance videos with GAN-based future frame prediction},
  author={Nguyen, Khac-Tuan and Dinh, Dat-Thanh and Do, Minh N and Tran, Minh-Triet},
  journal={Int. Conference on Multimedia Retrieval},
  pages={457--463},
  year={2020}
}

@article{crime,
  title={Suspicious Activity Detection in Surveillance Footage},
  author={Loganathan, Sathyajit and Kariyawasam, Gayashan and Sumathipala, Prasanna},
  journal={Int. Conference on Electrical and Computing Technologies and Applications},
  pages={1--4},
  year={2019},
  organization={IEEE}
}

@article{ucf_crime,
  title={Real-world anomaly detection in surveillance videos},
  author={Sultani, Waqas and Chen, Chen and Shah, Mubarak},
  journal={IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6479--6488},
  year={2018}
}

@article{anomaly_overview,
  title={An overview of deep learning based methods for unsupervised and semi-supervised anomaly detection in videos},
  author={Kiran, B Ravi and Thomas, Dilip Mathew and Parakkal, Ranjith},
  journal={Journal of Imaging},
  volume={4},
  number={2},
  pages={36},
  year={2018},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{enc_dec_multi_sensor,
  title={LSTM-based encoder-decoder for multi-sensor anomaly detection},
  author={Malhotra, Pankaj and Ramakrishnan, Anusha and Anand, Gaurangi and Vig, Lovekesh and Agarwal, Puneet and Shroff, Gautam},
  journal={arXiv preprint arXiv:1607.00148},
  year={2016}
}

@article{enc_dec_gan,
  title={Skip-ganomaly: Skip connected and adversarially trained encoder-decoder anomaly detection},
  author={Ak{\c{c}}ay, Samet and Atapour-Abarghouei, Amir and Breckon, Toby P},
  journal={International Joint Conference on Neural Networks (IJCNN)},
  pages={1--8},
  year={2019},
  organization={IEEE}
}

@article{mpedrnn,
  title={Learning regularity in skeleton trajectories for anomaly detection in videos},
  author={Morais, Romero and Le, Vuong and Tran, Truyen and Saha, Budhaditya and Mansour, Moussa and Venkatesh, Svetha},
  journal={IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11996--12004},
  year={2019}
}

@article{novelty_1,
  title={Novelty detection: a review—part 1: statistical approaches},
  author={Markou, Markos and Singh, Sameer},
  journal={Signal processing},
  volume={83},
  number={12},
  pages={2481--2497},
  year={2003},
  publisher={Elsevier}
}

@article{novelty_2,
  title={Novelty detection: a review—part 2:: neural network based approaches},
  author={Markou, Markos and Singh, Sameer},
  journal={Signal processing},
  volume={83},
  number={12},
  pages={2499--2521},
  year={2003},
  publisher={Elsevier}
}

@article{security_screening,
  title={Skip-ganomaly: Skip connected and adversarially trained encoder-decoder anomaly detection},
  author={Ak{\c{c}}ay, Samet and Atapour-Abarghouei, Amir and Breckon, Toby P},
  journal={2019 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--8},
  year={2019},
  organization={IEEE}
}

@article{real_world,
  title={Real-world anomaly detection in surveillance videos},
  author={Sultani, Waqas and Chen, Chen and Shah, Mubarak},
  journal={IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6479--6488},
  year={2018}
}

@article{any_shot,
  title={Any-shot sequential anomaly detection in surveillance videos},
  author={Doshi, Keval and Yilmaz, Yasin},
  journal={IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={934--935},
  year={2020}
}

@article{visual_attention,
  title={Deep anomaly detection through visual attention in surveillance videos},
  author={Nasaruddin, Nasaruddin and Muchtar, Kahlil and Afdhal, Afdhal and Dwiyantoro, Alvin Prayuda Juniarta},
  journal={Journal of Big Data},
  volume={7},
  number={1},
  pages={1--17},
  year={2020},
  publisher={SpringerOpen}
}

@article{billion_cameras,
  title={A world with a billion cameras watching you is just around the corner},
  author={Lin, Liza and Purnell, Newley},
  journal={The Wall Street Journal},
  year={2019}
}

@article{continual_learning,
  title={Continual learning for anomaly detection in surveillance videos},
  author={Doshi, Keval and Yilmaz, Yasin},
  journal={IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={254--255},
  year={2020}
}

@article{avenue,
  title={Abnormal event detection at 150 fps in matlab},
  author={Lu, Cewu and Shi, Jianping and Jia, Jiaya},
  journal={IEEE Int. Conference on computer vision},
  pages={2720--2727},
  year={2013}
}

@article{ucsd_ped2,
  title={Anomaly detection in crowded scenes},
  author={Mahadevan, Vijay and Li, Weixin and Bhalodia, Viral and Vasconcelos, Nuno},
  journal={IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1975--1981},
  year={2010},
  organization={IEEE}
}

@article{shaghai_tech,
  title={A revisit of sparse coding based anomaly detection in stacked rnn framework},
  author={Luo, Weixin and Liu, Wen and Gao, Shenghua},
  journal={IEEE Int. Conference on Computer Vision},
  pages={341--349},
  year={2017}
}

@article{hr_crime,
title = {HR-Crime: Human-Related Anomaly Detection in Surveillance Videos},
author = {Boekhoudt, Kayleigh and Matei, Alina and Aghaei, Maya and Talavera, Estefania},
year = {2021}
}


@article{sparse_unusual_events,
  title={Online detection of unusual events in videos via dynamic sparse coding},
  author={Zhao, Bin and Fei-Fei, Li and Xing, Eric P},
  journal={IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3313--3320},
  year={2011},
  organization={IEEE}
}

@article{opticalflow1,
  title={Anomaly detection in low quality traffic monitoring videos using optical flow},
  author={Zhou, Jin and Kwan, Chiman},
  journal={Pattern Recognition and Tracking XXIX},
  volume={10649},
  pages={106490F},
  year={2018},
  organization={International Society for Optics and Photonics}
}

@article{opticalflow2,
  title={Textures of optical flow for real-time anomaly detection in crowds},
  author={Ryan, David and Denman, Simon and Fookes, Clinton and Sridharan, Sridha},
  journal={IEEE Int. Conference on advanced video and signal based surveillance (AVSS)},
  pages={230--235},
  year={2011},
  organization={IEEE}
}

@article{oriented_gradients,
  title={Histograms of oriented gradients for human detection},
  author={Dalal, Navneet and Triggs, Bill},
  journal={IEEE computer society Conference on Computer Vision and Pattern Recognition},
  volume={1},
  pages={886--893},
  year={2005},
  organization={Ieee}
}

@article{deeplearning1,
  title={Learning temporal regularity in video sequences},
  author={Hasan, Mahmudul and Choi, Jonghyun and Neumann, Jan and Roy-Chowdhury, Amit K and Davis, Larry S},
  journal={IEEE Conference on Computer Vision and Pattern Recognition},
  pages={733--742},
  year={2016}
}

@article{deeplearning2,
  title={Joint detection and recounting of abnormal events by learning deep generic knowledge},
  author={Hinami, Ryota and Mei, Tao and Satoh, Shin'ichi},
  journal={IEEE Int. Conference on Computer Vision},
  pages={3619--3627},
  year={2017}
}

@article{futureframepred,
  title={Future frame prediction for anomaly detection--a new baseline},
  author={Liu, Wen and Luo, Weixin and Lian, Dongze and Gao, Shenghua},
  journal={IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6536--6545},
  year={2018}
}

@article{sparsecodingrnn,
  title={A revisit of sparse coding based anomaly detection in stacked rnn framework},
  author={Luo, Weixin and Liu, Wen and Gao, Shenghua},
  journal={IEEE Int. Conference on Computer Vision},
  pages={341--349},
  year={2017}
}

@article{improveddeeplearning,
  title={Improved anomaly detection in surveillance videos based on a deep learning method},
  author={Khaleghi, Ali and Moin, Mohammad Shahram},
  journal={Conference of AI \& Robotics and 10th RoboCup Iranopen International Symposium},
  pages={73--81},
  year={2018},
  organization={IEEE}
}

@article{motion_stats,
  title={Anomaly detection in surveillance video using motion direction statistics},
  author={Liu, Chang and Wang, Guijin and Ning, Wenxin and Lin, Xinggang and Li, Liang and Liu, Zhou},
  journal={IEEE Int. Conference on Image Processing},
  pages={717--720},
  year={2010},
  organization={IEEE}
}

@article{gans1,
  title={Ganomaly: Semi-supervised anomaly detection via adversarial training},
  author={Akcay, Samet and Atapour-Abarghouei, Amir and Breckon, Toby P},
  journal={Asian Conference on Computer Vision},
  pages={622--637},
  year={2018},
  organization={Springer}
}

@article{gans2,
  title={Abnormal event detection in videos using generative adversarial nets},
  author={Ravanbakhsh, Mahdyar and Nabi, Moin and Sangineto, Enver and Marcenaro, Lucio and Regazzoni, Carlo and Sebe, Nicu},
  journal={IEEE Int. Conference on Image Processing},
  pages={1577--1581},
  year={2017},
  organization={IEEE}
}

@article{lstm1,
  title={Remembering history with convolutional lstm for anomaly detection},
  author={Luo, Weixin and Liu, Wen and Gao, Shenghua},
  journal={IEEE Int. Conference on Multimedia and Expo},
  pages={439--444},
  year={2017},
  organization={IEEE}
}

@article{lstmcnn,
  title={CNN features with bi-directional LSTM for real-time anomaly detection in surveillance networks},
  author={Ullah, Waseem and Ullah, Amin and Haq, Ijaz Ul and Muhammad, Khan and Sajjad, Muhammad and Baik, Sung Wook},
  journal={Multimedia Tools and Applications},
  pages={1--17},
  year={2020},
  publisher={Springer}
}

@article{c3d_feat,
  title={Learning spatiotemporal features with 3d convolutional networks},
  author={Tran, Du and Bourdev, Lubomir and Fergus, Rob and Torresani, Lorenzo and Paluri, Manohar},
  journal={IEEE Int. Conference on Computer Vision},
  pages={4489--4497},
  year={2015}
}

@article{mil,
  title={A framework for multiple-instance learning},
  author={Maron, Oded and Lozano-P{\'e}rez, Tom{\'a}s},
  journal={Advances in Neural Information Processing Systems},
  pages={570--576},
  year={1998},
  publisher={Citeseer}
}

@article{distracted_driving,
  title={Driver anomaly detection: A dataset and contrastive learning approach},
  author={Kopuklu, Okan and Zheng, Jiapeng and Xu, Hang and Rigoll, Gerhard},
  journal={IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={91--100},
  year={2021}
}

@article{car_accidents,
  title={Cadp: A novel dataset for cctv traffic camera based accident analysis},
  author={Shah, Ankit Parag and Lamare, Jean-Bapstite and Nguyen-Anh, Tuan and Hauptmann, Alexander},
  journal={IEEE Int. Conference on Advanced Video and Signal Based Surveillance (AVSS)},
  pages={1--9},
  year={2018},
  organization={IEEE}
}

@article{intro_automatic_surveillance,
  title={Introduction to the special section on video surveillance},
  author={Collins, Robert T. and Lipton, Alan J and Kanade, Takeo},
  journal={IEEE Transactions on pattern analysis and machine intelligence},
  volume={22},
  number={8},
  pages={745--746},
  year={2000},
  publisher={IEEE}
}

@article{survaillance_speed,
  title={A video surveillance system for speed detection of vehicles and law enforcement using automatic number plate recognition},
  author={Bhargava, Kritika and Goyal, Dinesh},
  journal={International journal of research in Computer Engineering and Electronics},
  volume={3},
  year={2014}
}

@article{video_anomaly_detection_survey,
  author={Ramachandra, Bharathkumar and Jones, Michael and Vatsavai, Ranga Raju},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
  title={A Survey of Single-Scene Video Anomaly Detection}, 
  year={2020}}
  
@article{forensic_video_footage,
  title={Forensic image analysis--CCTV distortion and artefacts},
  author={Seckiner, Dilan and Mallett, Xanth{\'e} and Roux, Claude and Meuwly, Didier and Maynard, Philip},
  journal={Forensic science international},
  volume={285},
  pages={77--85},
  year={2018},
  publisher={Elsevier}
}

@article{surveillance_survey,
  title={Intelligent distributed surveillance systems: a review},
  author={Valera, Maria and Velastin, Sergio A},
  journal={IEE Proceedings-Vision, Image and Signal Processing},
  volume={152},
  number={2},
  pages={192--204},
  year={2005},
  publisher={IET}
}

@article{gmm,
  title={Gaussian Mixture Models.},
  author={Reynolds, Douglas A},
  journal={Encyclopedia of biometrics},
  volume={741},
  pages={659--663},
  year={2009},
  publisher={Berlin, Springer}
}

@article{iso_forest,
author={F. T. {Liu} and K. M. {Ting} and Z. {Zhou}},
journal={IEEE Int. Conference on Data Mining},
title={Isolation Forest},
year={2008},
pages={413-422},
doi={10.1109/ICDM.2008.17},
ISSN={2374-8486},
month={Dec},}

@article{agg,
  title={Modern hierarchical, agglomerative clustering algorithms},
  author={M{\"u}llner, Daniel},
  journal={arXiv preprint arXiv:1109.2378},
  year={2011}
}

@article{agg1,
  title={Methods of hierarchical clustering},
  author={Murtagh, Fionn and Contreras, Pedro},
  journal={arXiv preprint arXiv:1105.0121},
  year={2011}
}

@article{k_means,
  title={Some methods for classification and analysis of multivariate observations},
  author={MacQueen, James and others},
  journal={Berkeley symposium on mathematical statistics and probability},
  volume={1},
  number={14},
  pages={281--297},
  year={1967},
  organization={Oakland, CA, USA}
}

@article{smote,
  title={SMOTE: synthetic minority over-sampling technique},
  author={Chawla, Nitesh V and Bowyer, Kevin W and Hall, Lawrence O and Kegelmeyer, W Philip},
  journal={Journal of artificial intelligence research},
  volume={16},
  pages={321--357},
  year={2002}
}

@article{adasyn,
  title={ADASYN: Adaptive synthetic sampling approach for imbalanced learning},
  author={He, Haibo and Bai, Yang and Garcia, Edwardo A and Li, Shutao},
  journal={IEEE international joint conference on neural networks (IEEE world congress on computational intelligence)},
  pages={1322--1328},
  year={2008},
  organization={IEEE}
}

@article{silhouette,
  title={Silhouettes: a graphical aid to the interpretation and validation of cluster analysis},
  author={Rousseeuw, Peter J},
  journal={Journal of computational and applied mathematics},
  volume={20},
  pages={53--65},
  year={1987},
  publisher={Elsevier}
}

@article{iba,
  title={Index of balanced accuracy: A performance measure for skewed class distributions},
  author={Garc{\'\i}a, Vicente and Mollineda, Ram{\'o}n Alberto and S{\'a}nchez, Jos{\'e} Salvador},
  journal={Iberian conference on pattern recognition and image analysis},
  pages={441--448},
  year={2009},
  organization={Springer}
}

@article{gmean,
  title={Addressing the curse of imbalanced training sets: one-sided selection},
  author={Kubat, Miroslav and Matwin, Stan and others},
  journal={Int. Conference on Machine Learning},
  volume={97},
  pages={179--186},
  year={1997},
  organization={Citeseer}
}

@article{t-test,
  title={T test as a parametric statistic},
  author={Kim, Tae Kyun},
  journal={Korean journal of anesthesiology},
  volume={68},
  number={6},
  pages={540},
  year={2015},
  publisher={Korean Society of Anesthesiologists}
}

@article{relu,
  title={Searching for activation functions},
  author={Ramachandran, Prajit and Zoph, Barret and Le, Quoc V},
  journal={arXiv preprint arXiv:1710.05941},
  year={2017}
}

@article{adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{lstm,
  title={LSTM: A search space odyssey},
  author={Greff, Klaus and Srivastava, Rupesh K and Koutn{\'\i}k, Jan and Steunebrink, Bas R and Schmidhuber, J{\"u}rgen},
  journal={IEEE transactions on neural networks and learning systems},
  volume={28},
  number={10},
  pages={2222--2232},
  year={2016},
  publisher={IEEE}
}

@article{rnn_fundamentals,
  title={Fundamentals of recurrent neural network (RNN) and long short-term memory (LSTM) network},
  author={Sherstinsky, Alex},
  journal={Physica D: Nonlinear Phenomena},
  volume={404},
  pages={132306},
  year={2020},
  publisher={Elsevier}
}

@article{cross_entropy,
  title={Generalized cross entropy loss for training deep neural networks with noisy labels},
  author={Zhang, Zhilu and Sabuncu, Mert R},
  journal={arXiv preprint arXiv:1805.07836},
  year={2018}
}

@article{SHAPIRO1965,
  year  = {1965},
  month = {dec},
  publisher = {Oxford University Press ({OUP})},
  volume = {52},
  number = {3-4},
  pages = {591--611},
  author = {S. S. SHAPIRO and M. B. WILK},
  title = {An analysis of variance test for normality (complete samples)},
  journal = {Biometrika}
}

@article{hsu2005paired,
  title={Paired t test},
  author={Hsu, Henry and Lachenbruch, Peter A},
  journal={Encyclopedia of Biostatistics},
  volume={6},
  year={2005},
  publisher={Wiley Online Library}
}

@article{gehan1965generalized,
  title={A generalized Wilcoxon test for comparing arbitrarily singly-censored samples},
  author={Gehan, Edmund A},
  journal={Biometrika},
  volume={52},
  number={1-2},
  pages={203--224},
  year={1965},
  publisher={Oxford University Press}
}

@misc{chollet2015keras,
  title={Keras},
  author={Chollet, Fran\c{c}ois and others},
  year={2015},
  howpublished={\url{https://keras.io}},
}

@article{normalizing_flows,
  title={Anomaly detection in trajectory data with normalizing flows},
  author={Dias, Madson LD and Mattos, C{\'e}sar Lincoln C and da Silva, Ticiana LC and de Mac{\^e}do, Jos{\'e} Ant{\^o}nio F and Silva, Wellington CP},
  journal={International Joint Conference on Neural Networks (IJCNN)},
  pages={1--8},
  year={2020},
  organization={IEEE}
}

@article{gans,
  title={Coupled igmm-gans with applications to anomaly detection in human mobility data},
  author={Smolyak, Daniel and Gray, Kathryn and Badirli, Sarkhan and Mohler, George},
  journal={ACM Transactions on Spatial Algorithms and Systems},
  volume={6},
  number={4},
  pages={1--14},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@article{human_anomaly,
  title={Multi-camera open space human activity discovery for anomaly detection},
  author={Emonet, R{\'e}mi and Varadarajan, Jagannadan and Odobez, Jean-Marc},
  journal={IEEE Int. Conference on AVSS},
  year={2011},
}


@article{human_anomaly_1,
  title={Local distinguishability aggrandizing network for human anomaly detection},
  author={Gong, Maoguo and Zeng, Huimin and Xie, Yu and Li, Hao and Tang, Zedong},
  journal={Neural Networks},
  volume={122},
  pages={364--373},
  year={2020},
}

@article{human_activity,
  title={Human activity detection and recognition for video surveillance},
  author={Niu, Wei and Long, Jiao and Han, Dan and Wang, Yuan-Fang},
  journal={IEEE Int. Conference on multimedia and expo},
  volume={1},
  pages={719--722},
  year={2004},
  organization={IEEE}
}

@article{human_activity_1,
  title={Robust human activity recognition using multimodal feature-level fusion},
  author={Ehatisham-Ul-Haq, Muhammad and Javed, Ali and Azam, Muhammad Awais and Malik, Hafiz MA and Irtaza, Aun and Lee, Ik Hyun and Mahmood, Muhammad Tariq},
  journal={IEEE Access},
  volume={7},
  pages={60736--60751},
  year={2019},
  publisher={IEEE}
}

@article{human_activity_2,
  title={Activitynet: A large-scale video benchmark for human activity understanding},
  author={Caba Heilbron, Fabian and Escorcia, Victor and Ghanem, Bernard and Carlos Niebles, Juan},
  journal={IEEE Conference on Computer Vision and Pattern Recognition},
  pages={961--970},
  year={2015}
}

==> bibliowithpages.tex <==
@article{anomaly_survey,
  title={Anomaly detection: A survey},
  author={Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  journal={ACM computing surveys},
  volume={41},
  number={3},
  pages={1--58},
  year={2009},
  publisher={ACM New York, NY, USA}
}

@article{violence1,
  title={Violence detection in videos for an intelligent surveillance system using MoBSIFT and movement filtering algorithm},
  author={Febin, IP and Jayasree, K and Joy, Preetha Theresa},
  journal={Pattern Analysis and Applications},
  pages={1--13},
  year={2019},
  publisher={Springer}
}

@article{violence2,
  title={A new method for violence detection in surveillance scenes},
  author={Zhang, Tao and Yang, Zhijie and Jia, Wenjing and Yang, Baoqing and Yang, Jie and He, Xiangjian},
  journal={Multimedia Tools and Applications},
  volume={75},
  number={12},
  pages={7327--7349},
  year={2016},
  publisher={Springer}
}

@article{violence3,
  title={Human violence recognition and detection in surveillance videos},
  author={Bilinski, Piotr and Bremond, Francois},
  journal={ Int. Conference on Advanced Video and Signal Based Surveillance},
  pages={30--36},
  year={2016}
}

@article{car1,
  title={Motion interaction field for accident detection in traffic surveillance video},
  author={Yun, Kimin and Jeong, Hawook and Yi, Kwang Moo and Kim, Soo Wan and Choi, Jin Young},
  journal={Int. Conference on Pattern Recognition},
  pages={3062--3067},
  year={2014}
}

@article{car2,
  title={Anomaly detection in traffic surveillance videos with GAN-based future frame prediction},
  author={Nguyen, Khac-Tuan and Dinh, Dat-Thanh and Do, Minh N and Tran, Minh-Triet},
  journal={Int. Conference on Multimedia Retrieval},
  pages={457--463},
  year={2020}
}

@article{crime,
  title={Suspicious Activity Detection in Surveillance Footage},
  author={Loganathan, Sathyajit and Kariyawasam, Gayashan and Sumathipala, Prasanna},
  journal={Int. Conference on Electrical and Computing Technologies and Applications},
  pages={1--4},
  year={2019}
}

@article{ucf_crime,
  title={Real-world anomaly detection in surveillance videos},
  author={Sultani, Waqas and Chen, Chen and Shah, Mubarak},
  journal={ Conference on Computer Vision and Pattern Recognition},
  pages={6479--6488},
  year={2018}
}

@article{anomaly_overview,
  title={An overview of deep learning based methods for unsupervised and semi-supervised anomaly detection in videos},
  author={Kiran, B Ravi and Thomas, Dilip Mathew and Parakkal, Ranjith},
  journal={Journal of Imaging},
  volume={4},
  number={2},
  pages={36},
  year={2018},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{enc_dec_multi_sensor,
  title={LSTM-based encoder-decoder for multi-sensor anomaly detection},
  author={Malhotra, Pankaj and Ramakrishnan, Anusha and Anand, Gaurangi and Vig, Lovekesh and Agarwal, Puneet and Shroff, Gautam},
  journal={arXiv preprint arXiv:1607.00148},
  year={2016}
}

@article{enc_dec_gan,
  title={Skip-ganomaly: Skip connected and adversarially trained encoder-decoder anomaly detection},
  author={Ak{\c{c}}ay, Samet and Atapour-Abarghouei, Amir and Breckon, Toby P},
  journal={International Joint Conference on Neural Networks},
  pages={1--8},
  year={2019}
}

@article{mpedrnn,
  title={Learning regularity in skeleton trajectories for anomaly detection in videos},
  author={Morais, Romero and Le, Vuong and Tran, Truyen and Saha, Budhaditya and Mansour, Moussa and Venkatesh, Svetha},
  journal={Conference on Computer Vision and Pattern Recognition},
  pages={11996--12004},
  year={2019}
}

@article{novelty_1,
  title={Novelty detection: a review—part 1: statistical approaches},
  author={Markou, Markos and Singh, Sameer},
  journal={Signal processing},
  volume={83},
  number={12},
  pages={2481--2497},
  year={2003},
  publisher={Elsevier}
}

@article{novelty_2,
  title={Novelty detection: a review—part 2:: neural network based approaches},
  author={Markou, Markos and Singh, Sameer},
  journal={Signal processing},
  volume={83},
  number={12},
  pages={2499--2521},
  year={2003},
  publisher={Elsevier}
}

@article{security_screening,
  title={Skip-ganomaly: Skip connected and adversarially trained encoder-decoder anomaly detection},
  author={Ak{\c{c}}ay, Samet and Atapour-Abarghouei, Amir and Breckon, Toby P},
  journal={2019 International Joint Conference on Neural Networks},
  pages={1--8},
  year={2019}
}

@article{real_world,
  title={Real-world anomaly detection in surveillance videos},
  author={Sultani, Waqas and Chen, Chen and Shah, Mubarak},
  journal={ Conference on Computer Vision and Pattern Recognition},
  pages={6479--6488},
  year={2018}
}

@article{any_shot,
  title={Any-shot sequential anomaly detection in surveillance videos},
  author={Doshi, Keval and Yilmaz, Yasin},
  journal={Conference on Computer Vision and Pattern Recognition Workshops},
  pages={934--935},
  year={2020}
}

@article{visual_attention,
  title={Deep anomaly detection through visual attention in surveillance videos},
  author={Nasaruddin, Nasaruddin and Muchtar, Kahlil and Afdhal, Afdhal and Dwiyantoro, Alvin Prayuda Juniarta},
  journal={Journal of Big Data},
  volume={7},
  number={1},
  pages={1--17},
  year={2020},
  publisher={SpringerOpen}
}

@article{billion_cameras,
  title={A world with a billion cameras watching you is just around the corner},
  author={Lin, Liza and Purnell, Newley},
  journal={The Wall Street Journal},
  year={2019}
}

@article{continual_learning,
  title={Continual learning for anomaly detection in surveillance videos},
  author={Doshi, Keval and Yilmaz, Yasin},
  journal={Conference on Computer Vision and Pattern Recognition Workshops},
  pages={254--255},
  year={2020}
}

@article{avenue,
  title={Abnormal event detection at 150 fps in matlab},
  author={Lu, Cewu and Shi, Jianping and Jia, Jiaya},
  journal={ Int. Conference on computer vision},
  pages={2720--2727},
  year={2013}
}

@article{ucsd_ped2,
  title={Anomaly detection in crowded scenes},
  author={Mahadevan, Vijay and Li, Weixin and Bhalodia, Viral and Vasconcelos, Nuno},
  journal={ Conference on Computer Vision and Pattern Recognition},
  pages={1975--1981},
  year={2010}
}

@article{shaghai_tech,
  title={A revisit of sparse coding based anomaly detection in stacked rnn framework},
  author={Luo, Weixin and Liu, Wen and Gao, Shenghua},
  journal={ Int. Conference on Computer Vision},
  pages={341--349},
  year={2017}
}

@article{hr_crime,
title = {HR-Crime: Human-Related Anomaly Detection in Surveillance Videos},
author = {Boekhoudt, Kayleigh and Matei, Alina and Aghaei, Maya and Talavera, Estefania},
year = {2021}
}


@article{sparse_unusual_events,
  title={Online detection of unusual events in videos via dynamic sparse coding},
  author={Zhao, Bin and Fei-Fei, Li and Xing, Eric P},
  journal={ Conference on Computer Vision and Pattern Recognition},
  pages={3313--3320},
  year={2011}
}

@article{opticalflow1,
  title={Anomaly detection in low quality traffic monitoring videos using optical flow},
  author={Zhou, Jin and Kwan, Chiman},
  journal={Pattern Recognition and Tracking XXIX},
  volume={10649},
  year={2018},
  organization={International Society for Optics and Photonics}
}

@article{opticalflow2,
  title={Textures of optical flow for real-time anomaly detection in crowds},
  author={Ryan, David and Denman, Simon and Fookes, Clinton and Sridharan, Sridha},
  journal={ Int. Conference on advanced video and signal based surveillance},
  pages={230--235},
  year={2011}
}

@article{oriented_gradients,
  title={Histograms of oriented gradients for human detection},
  author={Dalal, Navneet and Triggs, Bill},
  journal={ computer society Conference on Computer Vision and Pattern Recognition},
  volume={1},
  pages={886--893},
  year={2005}
}

@article{deeplearning1,
  title={Learning temporal regularity in video sequences},
  author={Hasan, Mahmudul and Choi, Jonghyun and Neumann, Jan and Roy-Chowdhury, Amit K and Davis, Larry S},
  journal={ Conference on Computer Vision and Pattern Recognition},
  pages={733--742},
  year={2016}
}

@article{deeplearning2,
  title={Joint detection and recounting of abnormal events by learning deep generic knowledge},
  author={Hinami, Ryota and Mei, Tao and Satoh, Shin'ichi},
  journal={ Int. Conference on Computer Vision},
  pages={3619--3627},
  year={2017}
}

@article{futureframepred,
  title={Future frame prediction for anomaly detection--a new baseline},
  author={Liu, Wen and Luo, Weixin and Lian, Dongze and Gao, Shenghua},
  journal={ Conference on Computer Vision and Pattern Recognition},
  pages={6536--6545},
  year={2018}
}

@article{sparsecodingrnn,
  title={A revisit of sparse coding based anomaly detection in stacked rnn framework},
  author={Luo, Weixin and Liu, Wen and Gao, Shenghua},
  journal={ Int. Conference on Computer Vision},
  pages={341--349},
  year={2017}
}

@article{improveddeeplearning,
  title={Improved anomaly detection in surveillance videos based on a deep learning method},
  author={Khaleghi, Ali and Moin, Mohammad Shahram},
  journal={Conference of AI \& Robotics and 10th RoboCup Iranopen International Symposium},
  pages={73--81},
  year={2018}
}

@article{motion_stats,
  title={Anomaly detection in surveillance video using motion direction statistics},
  author={Liu, Chang and Wang, Guijin and Ning, Wenxin and Lin, Xinggang and Li, Liang and Liu, Zhou},
  journal={ Int. Conference on Image Processing},
  pages={717--720},
  year={2010}
}

@article{gans1,
  title={Ganomaly: Semi-supervised anomaly detection via adversarial training},
  author={Akcay, Samet and Atapour-Abarghouei, Amir and Breckon, Toby P},
  journal={Asian Conference on Computer Vision},
  pages={622--637},
  year={2018},
  organization={Springer}
}

@article{gans2,
  title={Abnormal event detection in videos using generative adversarial nets},
  author={Ravanbakhsh, Mahdyar and Nabi, Moin and Sangineto, Enver and Marcenaro, Lucio and Regazzoni, Carlo and Sebe, Nicu},
  journal={ Int. Conference on Image Processing},
  pages={1577--1581},
  year={2017}
}

@article{lstm1,
  title={Remembering history with convolutional lstm for anomaly detection},
  author={Luo, Weixin and Liu, Wen and Gao, Shenghua},
  journal={ Int. Conference on Multimedia and Expo},
  pages={439--444},
  year={2017}
}

@article{lstmcnn,
  title={CNN features with bi-directional LSTM for real-time anomaly detection in surveillance networks},
  author={Ullah, Waseem and Ullah, Amin and Haq, Ijaz Ul and Muhammad, Khan and Sajjad, Muhammad and Baik, Sung Wook},
  journal={Multimedia Tools and Applications},
  pages={1--17},
  year={2020},
  publisher={Springer}
}

@article{c3d_feat,
  title={Learning spatiotemporal features with 3d convolutional networks},
  author={Tran, Du and Bourdev, Lubomir and Fergus, Rob and Torresani, Lorenzo and Paluri, Manohar},
  journal={ Int. Conference on Computer Vision},
  pages={4489--4497},
  year={2015}
}

@article{mil,
  title={A framework for multiple-instance learning},
  author={Maron, Oded and Lozano-P{\'e}rez, Tom{\'a}s},
  journal={Advances in Neural Information Processing Systems},
  pages={570--576},
  year={1998},
  publisher={Citeseer}
}

@article{distracted_driving,
  title={Driver anomaly detection: A dataset and contrastive learning approach},
  author={Kopuklu, Okan and Zheng, Jiapeng and Xu, Hang and Rigoll, Gerhard},
  journal={Winter Conference on Applications of Computer Vision},
  pages={91--100},
  year={2021}
}

@article{car_accidents,
  title={Cadp: A novel dataset for cctv traffic camera based accident analysis},
  author={Shah, Ankit Parag and Lamare, Jean-Bapstite and Nguyen-Anh, Tuan and Hauptmann, Alexander},
  journal={ Int. Conference on Advanced Video and Signal Based Surveillance},
  pages={1--9},
  year={2018}
}

@article{intro_automatic_surveillance,
  title={Introduction to the special section on video surveillance},
  author={Collins, Robert T. and Lipton, Alan J and Kanade, Takeo},
  journal={ Transactions on pattern analysis and machine intelligence},
  volume={22},
  number={8},
  pages={745--746},
  year={2000}
}

@article{survaillance_speed,
  title={A video surveillance system for speed detection of vehicles and law enforcement using automatic number plate recognition},
  author={Bhargava, Kritika and Goyal, Dinesh},
  journal={International journal of research in Computer Engineering and Electronics},
  volume={3},
  year={2014}
}

@article{video_anomaly_detection_survey,
  author={Ramachandra, Bharathkumar and Jones, Michael and Vatsavai, Ranga Raju},
  journal={ Transactions on Pattern Analysis and Machine Intelligence}, 
  title={A Survey of Single-Scene Video Anomaly Detection}, 
  year={2020}
}
  
@article{forensic_video_footage,
  title={Forensic image analysis--CCTV distortion and artefacts},
  author={Seckiner, Dilan and Mallett, Xanth{\'e} and Roux, Claude and Meuwly, Didier and Maynard, Philip},
  journal={Forensic science international},
  volume={285},
  pages={77--85},
  year={2018},
  publisher={Elsevier}
}

@article{surveillance_survey,
  title={Intelligent distributed surveillance systems: a review},
  author={Valera, Maria and Velastin, Sergio A},
  journal={IEE Proceedings-Vision, Image and Signal Processing},
  volume={152},
  number={2},
  pages={192--204},
  year={2005},
  publisher={IET}
}

@article{gmm,
  title={Gaussian Mixture Models.},
  author={Reynolds, Douglas A},
  journal={Encyclopedia of biometrics},
  volume={741},
  pages={659--663},
  year={2009},
  publisher={Berlin, Springer}
}

@article{iso_forest,
author={F. T. {Liu} and K. M. {Ting} and Z. {Zhou}},
journal={ Int. Conference on Data Mining},
title={Isolation Forest},
year={2008},
pages={413-422},
doi={10.1109/ICDM.2008.17},
ISSN={2374-8486},
month={Dec},
}

@article{agg,
  title={Modern hierarchical, agglomerative clustering algorithms},
  author={M{\"u}llner, Daniel},
  journal={arXiv preprint arXiv:1109.2378},
  year={2011}
}

@article{agg1,
  title={Methods of hierarchical clustering},
  author={Murtagh, Fionn and Contreras, Pedro},
  journal={arXiv preprint arXiv:1105.0121},
  year={2011}
}

@article{k_means,
  title={Some methods for classification and analysis of multivariate observations},
  author={MacQueen, James and others},
  journal={Berkeley symposium on mathematical statistics and probability},
  volume={1},
  number={14},
  pages={281--297},
  year={1967},
  organization={Oakland, CA, USA}
}

@article{smote,
  title={SMOTE: synthetic minority over-sampling technique},
  author={Chawla, Nitesh V and Bowyer, Kevin W and Hall, Lawrence O and Kegelmeyer, W Philip},
  journal={Journal of artificial intelligence research},
  volume={16},
  pages={321--357},
  year={2002}
}

@article{adasyn,
  title={ADASYN: Adaptive synthetic sampling approach for imbalanced learning},
  author={He, Haibo and Bai, Yang and Garcia, Edwardo A and Li, Shutao},
  journal={ international joint conference on neural networks ( world congress on computational intelligence)},
  pages={1322--1328},
  year={2008}
}

@article{silhouette,
  title={Silhouettes: a graphical aid to the interpretation and validation of cluster analysis},
  author={Rousseeuw, Peter J},
  journal={Journal of computational and applied mathematics},
  volume={20},
  pages={53--65},
  year={1987},
  publisher={Elsevier}
}

@article{iba,
  title={Index of balanced accuracy: A performance measure for skewed class distributions},
  author={Garc{\'\i}a, Vicente and Mollineda, Ram{\'o}n Alberto and S{\'a}nchez, Jos{\'e} Salvador},
  journal={Iberian conference on pattern recognition and image analysis},
  pages={441--448},
  year={2009},
  organization={Springer}
}

@article{gmean,
  title={Addressing the curse of imbalanced training sets: one-sided selection},
  author={Kubat, Miroslav and Matwin, Stan and others},
  journal={Int. Conference on Machine Learning},
  volume={97},
  pages={179--186},
  year={1997},
  organization={Citeseer}
}

@article{t-test,
  title={T test as a parametric statistic},
  author={Kim, Tae Kyun},
  journal={Korean journal of anesthesiology},
  volume={68},
  number={6},
  pages={540},
  year={2015},
  publisher={Korean Society of Anesthesiologists}
}

@article{relu,
  title={Searching for activation functions},
  author={Ramachandran, Prajit and Zoph, Barret and Le, Quoc V},
  journal={arXiv preprint arXiv:1710.05941},
  year={2017}
}

@article{adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{lstm,
  title={LSTM: A search space odyssey},
  author={Greff, Klaus and Srivastava, Rupesh K and Koutn{\'\i}k, Jan and Steunebrink, Bas R and Schmidhuber, J{\"u}rgen},
  journal={ transactions on neural networks and learning systems},
  volume={28},
  number={10},
  pages={2222--2232},
  year={2016}
}

@article{rnn_fundamentals,
  title={Fundamentals of recurrent neural network (RNN) and long short-term memory (LSTM) network},
  author={Sherstinsky, Alex},
  journal={Physica D: Nonlinear Phenomena},
  volume={404},
  pages={132306},
  year={2020},
  publisher={Elsevier}
}

@article{cross_entropy,
  title={Generalized cross entropy loss for training deep neural networks with noisy labels},
  author={Zhang, Zhilu and Sabuncu, Mert R},
  journal={arXiv preprint arXiv:1805.07836},
  year={2018}
}

@article{SHAPIRO1965,
  year  = {1965},
  month = {dec},
  publisher = {Oxford University Press ({OUP})},
  volume = {52},
  number = {3-4},
  pages = {591--611},
  author = {S. S. SHAPIRO and M. B. WILK},
  title = {An analysis of variance test for normality (complete samples)},
  journal = {Biometrika}
}

@article{hsu2005paired,
  title={Paired t test},
  author={Hsu, Henry and Lachenbruch, Peter A},
  journal={Encyclopedia of Biostatistics},
  volume={6},
  year={2005},
  publisher={Wiley Online Library}
}

@article{gehan1965generalized,
  title={A generalized Wilcoxon test for comparing arbitrarily singly-censored samples},
  author={Gehan, Edmund A},
  journal={Biometrika},
  volume={52},
  number={1-2},
  pages={203--224},
  year={1965},
  publisher={Oxford University Press}
}

@misc{chollet2015keras,
  title={Keras},
  author={Chollet, Fran\c{c}ois and others},
  year={2015},
  howpublished={\url{https://keras.io}},
}

@article{normalizing_flows,
  title={Anomaly detection in trajectory data with normalizing flows},
  author={Dias, Madson LD and Mattos, C{\'e}sar Lincoln C and da Silva, Ticiana LC and de Mac{\^e}do, Jos{\'e} Ant{\^o}nio F and Silva, Wellington CP},
  journal={International Joint Conference on Neural Networks},
  pages={1--8},
  year={2020}
}

@article{gans,
  title={Coupled igmm-gans with applications to anomaly detection in human mobility data},
  author={Smolyak, Daniel and Gray, Kathryn and Badirli, Sarkhan and Mohler, George},
  journal={ACM Transactions on Spatial Algorithms and Systems},
  volume={6},
  number={4},
  pages={1--14},
  year={2020}
}

@article{human_anomaly,
  title={Multi-camera open space human activity discovery for anomaly detection},
  author={Emonet, R{\'e}mi and Varadarajan, Jagannadan and Odobez, Jean-Marc},
  journal={ Int. Conference on AVSS},
  year={2011}
}


@article{human_anomaly_1,
  title={Local distinguishability aggrandizing network for human anomaly detection},
  author={Gong, Maoguo and Zeng, Huimin and Xie, Yu and Li, Hao and Tang, Zedong},
  journal={Neural Networks},
  volume={122},
  pages={364--373},
  year={2020}
}

@article{human_activity,
  title={Human activity detection and recognition for video surveillance},
  author={Niu, Wei and Long, Jiao and Han, Dan and Wang, Yuan-Fang},
  journal={ Int. Conference on multimedia and expo},
  volume={1},
  pages={719--722},
  year={2004}
}

@article{human_activity_1,
  title={Robust human activity recognition using multimodal feature-level fusion},
  author={Ehatisham-Ul-Haq, Muhammad and Javed, Ali and Azam, Muhammad Awais and Malik, Hafiz MA and Irtaza, Aun and Lee, Ik Hyun and Mahmood, Muhammad Tariq},
  journal={ Access},
  volume={7},
  pages={60736--60751},
  year={2019},
}

@article{human_activity_2,
  title={Activitynet: A large-scale video benchmark for human activity understanding},
  author={Caba Heilbron, Fabian and Escorcia, Victor and Ghanem, Bernard and Carlos Niebles, Juan},
  journal={ Conference on Computer Vision and Pattern Recognition},
  pages={961--970},
  year={2015}
}

==> biography.tex <==
%{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{photos/}}
\bullet \textbf{MSc. Alina Matei} has obtained her Master's degree in Computer Science from University of Groningen, the Netherlands, in 2021. Her specialization field is software engineering, however, her interests also include computer vision and behaviour understanding. 

\bullet \textbf{Dr. Estefania Talavera} is currently an Assistant Professor at the University of Twente, The Netherlands. She obtained her PhD degree in Computer Science from the University of Groningen and the University of Barcelona in 2020. Her research interests are in learning-based approaches for behaviour understanding, data mining, and health applications.
    
\bullet \textbf{Dr. Maya Aghaei} is a Senior Researcher at the Computer Vision and Data Science professorship at NHLStenden University, Leeuwarden, The Netherlands. She is currently focused at applied research in the fields of Computer Vision, Machine Learning and Deep Learning. Her main topic of interests are Human-Human and Human-Computer Interaction analysis.


==> clustering_table.tex <==
\begin{table}[]
    \centering
%     \begin{tabular}{l|c}
% Unsupervised approach & Sillhouette score \\
% \hline \hline
% \textbf{Gmm} & \textbf{0.752} \\
% K-means clustering & \textbf{0.848} \\
% Isolation forest & 0.726 \\
% Agglomerative clustering & 0.846 \\
% \hline\hline
% Threshold = 0.0102 & 0.796 \\
% \end{tabular}


\resizebox{0.9\textwidth}{!}{\begin{tabular}{l|c|c|c}
% Unsupervised approach & \begin{rotate}{45} Sillhouette score \end{rotate} & \begin{rotate}{45} \#Normal to anomaly \end{rotate}  &  \begin{rotate}{45}\#Anomaly to normal \end{rotate}  \\
 & \begin{tabular}[c]{@{}c@{}}Silhouette score\\ \end{tabular}  & \begin{tabular}[c]{@{}c@{}}\#Abnormal \\ as wrongly normal\end{tabular}  &  \begin{tabular}[c]{@{}c@{}}\#Normal \\ as wrongly abnormal \end{tabular}  \\
\hline \hline
GMM & 0.752 & 24,549 & 11,748 \\
% K-means clustering & 0.848 & 24403 & 14380 \\
% Isolation forest & 0.726 & 24604 & 11846 \\
% Agglomerative clustering & 0.846 & 24405 & 14317 \\
\hline \hline
Threshold = 0.0102 & 0.796 & 24,533 & 11,987 \\
\end{tabular}}

    \caption{Silhouette score for the supervised and the unsupervised approaches after addressing the wrongly labeled `normal' and `abnormal' trajectories due to the original video-level annotation propagation. As a reference, the third column shows the number of trajectories that originally belonged to `normal' class and after thresholding are relabelled to `abnormal'.}
    \label{tab:clustering_ss}
\end{table}

==> end_to_end_14classes_topk.tex <==
\begin{table}[]
    \centering
\resizebox{0.5\textwidth}{!}{\begin{tabular}{ll||cc}
Model & Fusion & Top-3 accuracy & Top-5 accuracy \\
\hline \hline
\multicolumn{4}{c}{GMM}\\
\hline
softmax & late & 0.4182 $\pm$ 0.0146 & 0.5335 $\pm$ 0.0151 \\
conv1d & late & 0.3369 $\pm$ 0.0058 & 0.4420 $\pm$ 0.0077 \\
LSTM & late & 0.4107 $\pm$ 0.0159 & 0.5207 $\pm$ 0.0191 \\
conv1d & early (c) & 0.3815 $\pm$ 0.0132 & 0.5000 $\pm$ 0.0138 \\
conv1d & early (a) & 0.4499 $\pm$ 0.0178 & 0.5789 $\pm$ 0.0212 \\
\hline \hline
\multicolumn{4}{c}{threshold}\\
\hline
softmax & late & 0.3999 $\pm$ 0.0186 & 0.5168 $\pm$ 0.0215 \\
conv1d & late & 0.3704 $\pm$ 0.0055 & 0.4814 $\pm$ 0.0087 \\
LSTM & late & 0.3814 $\pm$ 0.0161 & 0.4813 $\pm$ 0.0116 \\
conv1d & early (c) & 0.3588 $\pm$ 0.0082 & 0.4678 $\pm$ 0.0092 \\
conv1d & early (a) & 0.3923 $\pm$ 0.0278 & 0.5072 $\pm$ 0.0305 \\
\end{tabular}}
    \caption{End to end 14 classes top k}
    \label{tab:my_label}
\end{table}

==> hierarchical.tex <==
\begin{table*}[!hbt]
    \centering
\resizebox{\textwidth}{!}{    \begin{tabular}{ll||cccccc}
Model ID & \begin{tabular}[c]{@{}l@{}}Data \\ augment. \end{tabular} & Accuracy (M) & Accuracy (W) & Precision (W) & Recall (W) & F-score (W) & IBA \\
\hline \hline
\multicolumn{8}{c}{GMM}\\
\hline
MPED-H1 & None & 0.551 & 0.256 & 0.686 & 0.551 & 0.594 & 0.501 \\
MPED-H2 & shift & \textcolor{blue}{0.527} & \textcolor{blue}{0.258} & \textcolor{blue}{0.691} & \textcolor{blue}{0.527} & \textcolor{blue}{0.584} & \textcolor{blue}{0.482} \\
\hline\hline
\multicolumn{8}{c}{Threshold}\\
\hline
MPED-H3 & None & 0.575 & 0.259 & 0.705 & 0.575 & 0.618 & 0.527 \\
MPED-H4 & shift & \textbf{\textcolor{orange}{0.581}} & \textbf{\textcolor{orange}{0.297}} & \textbf{\textcolor{orange}{0.722}} & \textbf{\textcolor{orange}{0.581}} & \textbf{\textcolor{orange}{0.629}} & \textbf{\textcolor{orange}{0.537}} \\
\end{tabular}}
    \caption{Results for the MPED-Hierarchical experiments; the MPED-Binary and MPED-Crime which constitute the hierarchical pipeline are based on Architecture C3 with 1D convolution layers; the data augmentation columns refers to the training dataset of MPED-Crime. Bold text identifies best performance per metric, highlighted text indicates models of interest for this study.}
    \label{tab:res_mped_hier}
\end{table*}

==> results_binary.tex <==
\begin{table}[]
    \centering
\resizebox{\textwidth}{!}{    \begin{tabular}{ll||cccccc}
Model ID & Fusion & Accuracy (M) & Accuracy (W)  & Precision (W) & Recall (W) & F-score (W) & IBA \\
\hline \hline
\multicolumn{8}{c}{GMM}\\
\hline
MPED-B1 & concat. & 0.789 $\pm$ 0.017 & 0.784 $\pm$ 0.019 & 0.791 $\pm$ 0.016 & 0.789 $\pm$ 0.017 & 0.788 $\pm$ 0.018 & 0.616 $\pm$ 0.029 \\
MPED-B2 & agg. & \textbf{\textcolor{blue}{0.808 $\pm$ 0.010}} & \textcolor{blue}{0.804 $\pm$ 0.012} & \textbf{\textcolor{blue}{0.810 $\pm$ 0.009}} & \textbf{\textcolor{blue}{0.808 $\pm$ 0.010}} & \textbf{\textcolor{blue}{0.807 $\pm$ 0.011}} & \textcolor{blue}{0.647 $\pm$ 0.019} \\

\hline \hline
\multicolumn{8}{c}{Threshold}\\
\hline
MPED-B3 & concat. & 0.805 $\pm$ 0.005 & 0.802 $\pm$ 0.005 & 0.806 $\pm$ 0.006 & 0.805 $\pm$ 0.005 & 0.804 $\pm$ 0.005 & 0.644 $\pm$ 0.009 \\
MPED-B4 & agg. & \textcolor{orange}{0.806 $\pm$ 0.005} & \textbf{\textcolor{orange}{0.805 $\pm$ 0.006}} & \textcolor{orange}{0.806 $\pm$ 0.005} & \textcolor{orange}{0.806 $\pm$ 0.005} & \textcolor{orange}{0.806 $\pm$ 0.005} & \textbf{\textcolor{orange}{0.648 $\pm$ 0.009}} 

\end{tabular}}
    \caption{Results for the MPED-Binary experiments on different types of early fusion (aggregation or concatenation); the MPED-Binary models is based on 1D convolution layers as shown in Figure \ref{fig:mped_C_model}. Bold text identifies best performance per metric, highlighted text indicates models of interest for this study.}
    \label{tab:res_mped_binary}
\end{table}

==> results_end_to_end_topk.tex <==
\begin{table}[]
    \centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lll||cc}
Model & Data aug. & Fusion & Top-3 accuracy & Top-5 accuracy \\
\hline \hline
\multicolumn{5}{c}{GMM} \\
\hline
softmax & None & late & 0.6771 $\pm$ 0.0050 & 0.8248 $\pm$ 0.0055 \\
% softmax & shift & late & 0.6423 $\pm$ 0.0137 & 0.7996 $\pm$ 0.0173 \\
softmax & None & late & 0.5707 $\pm$	0.0048 &	0.7493 $\pm$	0.0019\\
conv1d & None & late & 0.7059 $\pm$ 0.0069 & 0.8391 $\pm$ 0.0032 \\
% conv1d & shift & late & 0.6859 $\pm$ 0.0061 & 0.8341 $\pm$ 0.0031 \\
conv1d & shift & late & 0.6212 $\pm$	0.0167 & 0.7967 $\pm$	0.0101\\
LSTM & None & late & 0.7005 $\pm$ 0.0052 & 0.8372 $\pm$ 0.0035 \\
% LSTM & shift & late & 0.6863 $\pm$ 0.0055 & 0.8332 $\pm$ 0.0032 \\
LSTM & shift & late & 0.6329 $\pm$	0.0135 &	0.8023 $\pm$	0.0091\\
conv1d & None & early (c) & 0.7137 $\pm$ 0.0072 & 0.8496 $\pm$ 0.0031 \\
% conv1d & shift & early (c) & 0.6985 $\pm$ 0.0124 & 0.8389 $\pm$ 0.0068 \\
conv1d & shift & early (c) & 0.6604 $\pm$ 0.0030 & 0.8202 $\pm$ 0.0002\\
conv1d & None & early (a) & 0.7182 $\pm$ 0.0016 & 0.8500 $\pm$ 0.0023 \\
% conv1d & shift & early (a) & 0.7182 $\pm$  0.0016 & 0.8500 $\pm$ 0.0023 \\
conv1d & shift & early (a) & 0.6588 $\pm$ 0.0028 &	0.8162 $\pm$	0.0026\\
\hline \hline
\multicolumn{5}{c}{threshold} \\
\hline
softmax & None & late & 0.6547 $\pm$ 0.0050 & 0.8149 $\pm$ 0.0052 \\
% softmax & shift & late & 0.6495 $\pm$ 0.0023 & 0.8135 $\pm$ 0.0052 \\
softmax & shift & late & 0.5769	$\pm$ 0.0079 & 0.7589 $\pm$	0.0072\\
conv1d & None & late & 0.6898 $\pm$ 0.0125 & 0.8344 $\pm$ 0.0079 \\
% conv1d & shift & late & 0.6776 $\pm$ 0.0102 & 0.6776 $\pm$ 0.0056 \\
conv1d & shift & late & 0.6338 $\pm$ 0.0161 & 0.7984 $\pm$ 0.0090\\
LSTM & None & late & 0.6883 $\pm$ 0.0073 & 0.8300 $\pm$ 0.0050 \\
% LSTM & shift & late & 0.6806 $\pm$	0.0114 &	0.8254 $\pm$	0.0045\\
LSTM & shift & late & 0.6575 $\pm$ 0.0061 & 0.8116 $\pm$ 0.0024\\
conv1d & None & early (c) & 0.7109 $\pm$ 0.0063 & 0.8397 $\pm$ 0.0028 \\
% conv1d & shift & early (c) & 0.7072 $\pm$ 0.0031 & 0.7072 $\pm$ 0.0024 \\
conv1d & shift & early (c) & 0.6669 $\pm$ 0.0120 & 0.8185 $\pm$ 0.0084\\
conv1d & None & early (a) & 0.7106 $\pm$ 0.0036 & 0.8414 $\pm$ 0.0036 \\
% conv1d & shift & early (a) & 0.6930 $\pm$ 0.0192 & 0.8345 $\pm$ 0.0124 \\
conv1d & shift & early (a) & 0.6502	$\pm$ 0.0147 & 0.8045 $\pm$ 0.0051\\
\end{tabular}}
    \caption{End-to-end results top acc 13 crimes}
    \label{tab:my_label}
\end{table}

==> results_rec_classifiers_topk.tex <==
\begin{table}[h]
    \centering
    
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lll||cc}
Model ID & Ground truth & Data augmentation & Top-3 accuracy & Top-5 accuracy  \\
\hline \hline
M1.1 & k-means & None & 0.686 $\pm$ 0.002 & 0.860 $\pm$ 0.005 \\
M1.2 & k-means & SMOTE & 0.640 $\pm$ 0.002 & 0.881 $\pm$ 0.007 \\

M2.1 & isolation forest & None & 0.615 $\pm$ 0.002 & 0.838 $\pm$ 0.002 \\
M2.2 & isolation forest & SMOTE & 0.574 $\pm$ 0.006 & 0.823 $\pm$ 0.006 \\

M3.1 & GMM & None & 0.629 $\pm$ 0.007 & 0.861 $\pm$ 0.004 \\
M3.2 & \textcolor{blue}{GMM} & \textcolor{blue}{SMOTE} & \textcolor{blue}{0.577 $\pm$ 0.010} & \textcolor{blue}{0.846 $\pm$ 0.003} \\

M4.1 & agglomerative & None & 0.630 $\pm$ 0.009 & 0.830 $\pm$ 0.004 \\
M4.2 & agglomerative & SMOTE & 0.563 $\pm$ 0.009 & 0.834 $\pm$ 0.005 \\
\hline \hline
M5.1 & threshold & None & 0.642 $\pm$ 0.006 & 0.855 $\pm$ 0.005 \\
M5.2 & threshold & SMOTE & 0.596 $\pm$ 0.004 & 0.843 $\pm$ 0.004 \\
\end{tabular}}
    \caption{Top-3 and Top-5 accuracy results for the 13 crimes classifiers; this Table completes the results showcased in Table \ref{tab:res_13classifier}.}
    \label{tab:topk_13classifier}
\end{table}



==> stats_MPEDCrime.tex <==
\begin{table*}[!ht]
    \centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{cc||cc}
Model 1 ID & Model 2 ID & Normality test value & P-value \\
\hline \hline
MPED-C5.2 & MPED-C4.2 & 0.319 &  0.778 \\
MPED-C5.2 & MPED-C10.2 & 0.616 & 0.083 \\
MPED-C5.2 & MPED-C8.2 & 0.869 &  0.415 \\
MPED-C5.2 & MPED-C9.2 & 0.473 &  0.153 \\
MPED-C5.2 & MPED-C3.2 & 0.760 &  0.151 \\
\end{tabular}}

    \caption{Results of statistical test comparing the top-6 best performing experiments in Table \ref{tab:res_mped_crime} for the MPED-Crime model}
    \label{tab:stats_mped_crime}
\end{table*}


% \begin{tabular}{cc||ccc}
% Model 1 ID & Model 2 ID & Normality test value & Statistical test & P-value \\
% \hline \hline
% MPED-C5.2 & MPED-C4.2 & 0.319 & t-test & 0.778 \\
% MPED-C5.2 & MPED-C10.2 & 0.616 & t-test & 0.083 \\
% MPED-C5.2 & MPED-C8.2 & 0.869 & t-test & 0.415 \\
% MPED-C5.2 & MPED-C9.2 & 0.473 & t-test & 0.153 \\
% MPED-C5.2 & MPED-C3.2 & 0.760 & t-test & 0.151 \\
% \end{tabular}

==> stats_MPEDNormalCrime.tex <==
\begin{table*}[]
    \centering
\resizebox{0.7\textwidth}{!}{  \begin{tabular}{ll||ccc}
Model 1 & Model 2 & Normality test value & P-value \\
\hline \hline
MPED-NC5 & MPED-NC3 & 0.809  & 0.451 \\
MPED-NC5 & MPED-NC10 & 0.522  & 0.683 \\
MPED-NC5 & MPED-NC9 & 0.729 & 0.027 \\
MPED-NC5 & MPED-NC4 & 0.843 & 0.198 \\
MPED-NC5 & MPED-NC8 & 0.546 & 0.154 \\
\end{tabular} }
    \caption{Results of statistical test comparing the top-6 best performing experiments in Table \ref{tab:res_mped_nc} for the MPED-NormalCrime model}
    \label{tab:stats_mped_nc}
\end{table*}


% \begin{tabular}{ll||ccc}
% Model 1 & Model 2 & Normality test value & Statistical test & P-value \\
% \hline \hline
% MPED-NC5 & MPED-NC3 & 0.809 & t-test & 0.451 \\
% MPED-NC5 & MPED-NC10 & 0.522 & t-test & 0.683 \\
% MPED-NC5 & MPED-NC9 & 0.729 & t-test & 0.027 \\
% MPED-NC5 & MPED-NC4 & 0.843 & t-test & 0.198 \\
% MPED-NC5 & MPED-NC8 & 0.546 & t-test & 0.154 \\
% \end{tabular}

==> stats_res13.tex <==
\begin{table*}[ht]
    \centering
\resizebox{.6\textwidth}{!}{  
\begin{tabular}{cc||cc}
Model 1 ID & Model 2 ID & Normality Test Value & P value \\
\hline \hline
M1.2 & M2.2 & 0.525 & 0.056 \\
M1.2 & M1.1 & 0.053 & 0.001 \\
M1.2 & M2.1 & 0.030 & 0.109 \\
\end{tabular} }
    \caption{Results of statistical tests comparing the experiments in Table \ref{tab:res_13classifier} for the decoded-based classification models.}
    \label{tab:stats_13classifier}
\end{table*}

% \begin{tabular}{cc||ccc}
% Model 1 ID & Model 2 ID & Normality Test Value & Type of Statistical Test & P value \\
% \hline \hline
% M3.2 & M5.2 & 0.525 & T-test & 0.056 \\
% M3.2 & M2.2 & 0.385 & T-test & 0.005 \\
% M3.2 & M1.2 & 0.231 & T-test & 0.008 \\
% M3.2 & M3.1 & 0.053 & T-test & 0.001 \\
% M3.2 & M5.1 & 0.030 & Wilcoxon & 0.109 \\
% \end{tabular}

==> top5_13crimes.tex <==
\begin{table*}[!hbt]
    \centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l}
\textit{Abuse} & \textit{Arrest} & \textit{Arson} & \textit{Assault} & \textit{Burglary} & \textit{Explosion} & \textit{Fighting} & \textit{Road Accidents} & \textit{Robbery} & \textit{Shooting} & \textit{Shoplifting} & \textit{Stealing} & \textit{Vandalism} \\
\hline \hline
\textbf{Abuse} & \textbf{Arrest} & \textbf{Arson} & \textbf{Assault} & \textbf{Burglary} & Shooting & \textbf{Fighting} & \textbf{R. Accidents} & \textbf{Robbery} & \textbf{Shooting} & \textbf{Shoplifting} & \textbf{Stealing} & Fighting \\
Fighting & Fighting & Assault & Fighting & Fighting & Fighting & Assault & Fighting & Shoplifting & Fighting & Robbery & Fighting & \textbf{Vandalism} \\
Shoplifting & Assault & Fighting & Robbery & Arrest & \textbf{Explosion} & Arrest & Assault & Assault & Arrest & Fighting & Assault & Burglary \\
Burglary & Burglary & Burglary & Burglary & Assault & Stealing & Stealing & Shooting & Fighting & Arson & Assault & Arson & Stealing \\
Assault & Robbery & Robbery & Arrest & Shoplifting & Arrest & Arson & Burglary & Burglary & Assault & Burglary & R. Accidents & Arrest \\
\end{tabular}}


    \caption{Top-5 predictions for the crimes classifier with ID M1.2, proposed in Section \ref{sec:decoded_based_classif}.}
    \label{tab:most_common_preds_13crimes}
\end{table*}
